Efficient Anomaly Detection via Matrix Sketching

We consider the problem of finding anomalies in high-dimensional data using popular PCA based anomaly scores. The naive algorithms for computing these scores explicitly compute the PCA of the covariance matrix which uses space quadratic in the dimensionality of the data. We give the first streaming algorithms that use space that is linear or sublinear in the dimension. We prove general results showing that \emph{any} sketch of a matrix that satisfies a certain operator norm guarantee can be used to approximate these scores. We instantiate these results with powerful matrix sketching techniques such as Frequent Directions and random projections to derive efficient and practical algorithms for these problems, which we validate over real-world data sets. Our main technical contribution is to prove matrix perturbation inequalities for operators arising in the computation of these measures.

==> abstract.tex <==
\begin{abstract}
We present efficient streaming algorithms to compute two commonly used
anomaly measures: the rank-$k$ leverage scores (aka Mahalanobis
distance) and the rank-$k$ projection distance, in the row-streaming
model. We show that commonly used matrix sketching techniques
such as the  Frequent Directions sketch and random projections can be used
to approximate these measures. Our main technical contribution is to
prove matrix perturbation inequalities for operators arising in the
computation of these measures.
\end{abstract}

%\begin{keywords}
%anomaly detection, leverage scores, matrix perturbation, %Mahalanobis distance, covariance estimation
%\end{keywords}


==> batch.tex <==



\eat{



We will use the following simple Lemma to bound the sum of absolute
values of diagonal entries in symmetric matrices.
\begin{lemma}\label{lem:tr_abs}
   Let $\Ab \in \R^{n \times n}$ be symmetric. Then
   \[ \sum_{i=1}^{n}\Big| {\eb_i^T\Ab \eb_i}\Big| \leq \rk(\Ab)\|\Ab\|. \]
 \end{lemma}
 \begin{proof}
 	Consider the eigenvalue decomposition of $\Ab=\Qb \Lambdab \Qb^T$ where $\Lambdab$ is the diagonal matrix of eigenvalues of $\Ab$. We can write,
 	\begin{align*}
 	  \sum_{i=1}^{n}\Big| {\eb_i^T\Ab \eb_i}\Big|
          & = \sum_{i=1}^{n}\Big| {\eb_i^T\Qb \Lambdab \Qb^T
            \eb_i}\Big| = \sum_{i=1}^{n}\Big| \Lambdab_{j,j}\Qb_{i,j}^2\Big| \\
 	  & \le \norm{\Ab} \sum_{i=1}^{n}\Big| \Qb_{i,j}^2\Big|  =
          \norm{\Ab} \normfsq{\Qb} = \rk(\Ab)\norm{\Ab}.
 	\end{align*}
 \end{proof}



\begin{lemma}
  \label{lem:batch-mhnbs}
  Let $\Ab \in \R^{n \times d}$ satisfy $\sigma^2_k(\Ab) - \sigma_{k+1}^2(\Ab)
  \geq \Delta \sigma_1^2(\Ab)$.  Let $\Bb \in \R^{\ell \times d}$ be such
    that
    \[ \norm{\Ab\Ab^T - \td{\Ab}\td{\Ab}^T} \leq \mu \sigma_1(\Ab)^2 \]
    where $\mu \leq \Delta/6$.
    Let $\Ab = \Ub_k\Sigma_k\Vb_k^T$ and $\Bb =
    \tilde{\Ub}_k\tilde{\Sigma}_k\tilde{\Vb}_k^T$ be their respective
    SVDs. Then
    \[ \sum_{i=1}^n |e_i^t\Ub_k\Ub_k^Te_i - e_i^t\tilde{\Ub}_k\tilde{\Ub}_k^Te_i| \leq 2\sqrt{\frac{\mu}{\Delta}}k.\]
\end{lemma}
\begin{proof}
  Let us define $\Cb = \Ub_k\Ub^T_k -
  \tilde{\Ub}_k\tilde{\Ub}_k^T$. So we have $\rank(\Cb) \leq 2k$. By
  Lemma \ref{lem:wed}, we have
  \[ \norm{\Cb} \leq 2\sqrt{\frac{\mu}{\Delta}}.\]
  So applying Lemma \ref{lem:tr_abs}, we get the desired bound.
\end{proof}

\begin{lemma}
  \label{lem:batch-proj}
    Let $\Ab \in \R^{n \times d}$ satisfy $\sigma^2_k(\Ab) - \sigma_{k+1}^2(\Ab)
  \geq \Delta \sigma_1^2(\Ab)$.  Let $\td{\Ab} \in \R^{\ell \times d}$ be such
    that
    \[ \norm{\Ab\Ab^T - \td{\Ab}\td{\Ab}^T} \leq \mu \sigma_1(\Ab)^2 \]
    where $\mu \leq \min(\Delta^3k^2, 1/(20 k))$.
    Let $\Ab = \Ub_k\Sigmab_k\Vb_k^T$ and $\td{\Ab} =
    \tilde{\Ub}_k\tilde{\Sigmab}_k\tilde{\Vb}_k^T$ be their respective
    SVDs. Then
    \[ \sum_{i=1}^n |e_i^t\Ub_k\Sigmab_k^2\Ub_k^Te_i -
    e_i^t\tilde{\Ub}_k\tilde{\Sigmab}_k^2\tilde{\Ub}_k^Te_i| \leq
    5\sigma(\Ab)^2\mu^{1/3}k^{4/3}.\]
\end{lemma}
\begin{proof}
  Let $\Cb = \Ub_k\Sigmab_k^2\Ub_k^T -
  \tilde{\Ub}_k\tilde{\Sigmab}_k^2\tilde{\Ub}_k^T$. It is easy to see
  that $\rank(\Cb) \leq 2k$. We now bound its operator norm as follows
  \begin{align*}
    \norm{\Cb} \leq \norm{\Ub_k\Sigmab_k^2\Ub_k^T -
      \tilde{\Ub}_k\Sigmab_k^2\tilde{\Ub}_k^T} + \norm{
      \tilde{\Ub}_k(\Sigmab_k^2 - \tilde{\Sigmab}_k^2)\tilde{\Ub}_k^T}.
  \end{align*}
  To bound the first term, we use Lemma \ref{lem:sigma1}:
  \[ \norm{\Ub_{\leq k}\Sigmab_k^2\Ub^t_{\leq k} - \tilde{\Ub}_{\leq
      k}\Sigmab_k^2\tilde{\Ub}^t_{\leq k}} \leq 4\sigma_1(\Ab)^2(\mu
  k)^{1/3}.\]
  For the second term, we use
  \[ \norm{\tilde{\Ub}_k(\Sigmab_k^2 -
    \tilde{\Sigmab}_k^2)\tilde{\Ub}_k^T} \leq \norm{\Sigmab_k^2 -
      \tilde{\Sigmab}_k^2} \leq \mu \sigma_1(\Ab)^2.
  \]
  Overall, we get $\norm{\Cb} \leq 5\sigma(\Ab)^2(\mu k)^{1/3}$. So
  applying Lemma \ref{lem:tr_abs}, we get
    \[ \sum_{i=1}^n |e_i^t\Ub_k\Sigmab_k^2\Ub_k^Te_i -
    e_i^t\tilde{\Ub}_k\tilde{\Sigmab}_k^2\tilde{\Ub}_k^Te_i| \leq
    5\sigma(\Ab)^2(\mu k)^{1/3} \cdot 2k \leq 5\sigma(\Ab)^2\mu^{1/3}k^{4/3}.\]
\end{proof}
}


==> intro_old.tex <==
\section{Introduction}

The goal of this paper is to provide efficient algorithms for anomaly detection for extremely high dimensional data.
Anomaly detection in high-dimensional numeric data is a ubiquitous
problem in machine learning \citep{Aggarwal2013,ChandolaBK09}. A typical scenario, which is the main motivation for this work, is where we have a
constant stream of measurements (say various parameters regarding the
health of machines in a data-center), and our goal is to detect any unusual
behavior. In such settings, labels are usually hard to come by and
unsupervised learning methods are preferred: the algorithm needs to learn what
the bulk of the data look like and then detect any deviations from this.

Any algorithm to detect anomalies in this setting faces computational
challenges: first, the dimension of the data may be very large, both
in terms of the number of data points and their dimensionality. In the
context of a data center there could be $10^4$ measurements per
machine and thousands of machines. In the context of IoT the number of
collecting devices may explode. Second, the distributed nature of this
setting suggests that storing the entire data, let alone transmitting
it in its entirety may be unfeasible.


There is no single definition of an anomaly. For instance,
clearly a data point which is unusual in magnitude should be
considered anomalous. A more subtle notion of anomalies are those that
stem from changes in the correlation  across dimensions. Consider for
instance the case where the CPU usage of a machine rises by
$10\%$. That in itself may not be considered an anomaly, however when
a large fraction of machines in the data center see this behavior
simultaneously an alarm should be issued. Another more subtle scenario
is when, say, a group of servers that are typically correlated
suddenly demonstrate uncorrelated changes in load. Detecting these
types of behaviors requires a more sophisticated way of assigning an
\emph{anomaly score} to a data point. We focus on two commonly used measures.

The Mahalanobis distance~\citep{Mahalanobis36} is well known  and
heavily used way to measure this type of anomaly\footnote{See
  \citet{Wilks63,Hawkins74} for classic uses of the Mahalanobis
  distance in statistical outlier detection.}. It relies on the
Singular Value Decomposition of the data matrix, the rows of the
matrix are data points and columns are types of measurements.

To define it formally, we need some notation. Given a matrix $\Ab \in
\R^{n \times d}$, we let $\rowa{i} \in \R^d$ denote its
$i^{th}$ row and $\cola{i} \in \R^n$ denote its $i^{th}$ column. We
consider all vectors as column vectors (that includes $\rowa{i}$).

\begin{Def}
Let $\Ab \in \R^{n \times d}$.  Let $\Ub \Sigmab \Vb^T$ be its SVD where
$\Sigmab = \diag(\sigma_1, \ldots, \sigma_d)$, for $\sigma_1 \geq
\cdots \geq \sigma_d > 0$. The Mahalanobis distance of the $i^{th}$
row is denoted $L(i)$ and is defined as,
\[ L(i) = \sum_{i=1}^d \frac{(\rowa{i}^T\colof{v}{i})^2}{\sigma^2_i}, \]
where $\rowa{i}$ and $\colof{v}{i}$ are the $i^{th}$ row of $\Ab$ and
$i^{th}$ column of $\Vb$ respectively. Equivalently, $L(i) =
\sqnorm{\rowof{u}{i}}$ where $u_{(i)}$ is the $i^{th}$ row of $\Ub$.
\end{Def}
$L(i)$ is also known as the  \emph{leverage score} \citep{Drineas12,Mahoney11}.
$L(i)$  depends on the entire spectrum of singular values and is clearly
very sensitive to smaller singular values. Many high dimensional data
sets arising in practice are close to being low-dimensional. The low
part of the spectrum might come from noise. In this case, the high
sensitivity to small singular values is undesirable.
A common approach to circumvent this is to limit the above sum for
only the $k$ largest singular values (for some appropriately chosen
$k \ll d$) \citep{Aggarwal2013, Holgersson12}.  This measure is called
the rank $k$ leverage score, and denoted by $L^k(i)$.
\[ L^k(i) = \sum_{i=1}^k \frac{(\rowa{i}^T\colof{v}{i})^2}{\sigma^2_i}. \]

The rank $k$ leverage score is concerned with the mass which lies
within the principal space. The  principal subspace represents what is
``normal'', and so we also need to catch the anomalies that are far
from it. To that end a second measure of anomaly is the
rank $k$ \emph{projection distance} of a point, which is simply the distance of
the data point $a_{(i)}$ to the rank $k$ principal subspace, and
denote this by $T^k(i)$. It is defined as
\[ T^k(i) = \sum_{i = k + 1}^d (\rowa{i}^T\colof{v}{i})^2. \]
This measure has been studied extensively and shown to be effective in practice, see
\citet{Huang15} and references therein. It presents a more stable
alternative to taking the {\em tail} of the Mahalanobis distance,
\[ L^{> k} (i) = \sum_{i=k+1}^d \frac{(\rowa{i}^T\colof{v}{i})^2}{\sigma^2_i}. \]

These two measures, the rank $k$ leverage scores and projection
distances are the focus of our work. We should note that many other
measures are  studied in the literature, such as the regularized (or soft)
Mahalanobis distance~\citep{Aggarwal2013}, also known as ridge
leverage~\citep{Holgersson12,Alaoui15,CohenMM17}. We discuss ridge
leverage scores in greater detail in  Section~\ref{sec:ridge}, and
show that in some settings, the ridge leverage
score can be viewed as a combination of $L^k(i)$ and $T^k(i)$.

\paragraph{The separation assumption}

Intuitively once $k$ is chosen it should determine the subspace which
approximates the data. However, if there is degeneracy in the spectrum
of the matrix, namely that  $\sigma_k^2 = \sigma_{k+1}^2$ then
$k$-dimensional principal subspace is not unique, and then
the quantities $L^k$ and $T^k$ are not well defined, since their value will
depend on the choice of principal subspace. This suggests that we are
using the {\em wrong} value of $k$, since the choice of $k$ ought to be
such that the directions orthogonal to the principal subspace have
markedly less variance than those in the principal subspace.
Hence  we require that $k$ is such that there
is a gap in the spectrum at $k$, which ensures that the principal
subspace is well defined.
\begin{Def}
\label{def:sep}
  A matrix $\Ab$ is $(k, \Delta)$-separated if
  \begin{align}
    \sigma_k^2 - \sigma^2_{k+1} \geq \Delta \sigma_1^2.
  \end{align}
\end{Def}
All our results assume that the data are $(k,\Delta)$-separated for
$\Delta > 0$, this assumptions manifests itself as an inverse polynomial dependence on
$\Delta$ in our bounds. We stress that this assumption is very
reasonable for real-life data sets.

\paragraph{The low stable rank assumption} We denote by $\|\Ab\|_F$ the Frobenius norm of the matrix, and by  $\|\Ab\|$ the operator norm (which is equal to the largest singular value).  Define the stable rank $\sr(\Ab)=\normfsq{\Ab}/\norm{\Ab}^2$. While it is not strictly needed, the reader should have in mind
the scenario where the top-$k$ principal subspace captures a constant
fraction (at least $0.5$) of the total variance in the data. This is
the setting where the measures $L^k$ and $T^k$ are meaningful. Note
that this assumption implies that the stable rank $\sr(\Ab) = O(k)$,
since $k\sigma_1^2$ is a constant fraction of the total Frobenius norm.

\paragraph{Online vs batch anomaly detection}
In our definition of leverage scores, we have assumed that the entire
matrix is  given to us as input. We refer to this as the batch
scenario. In practice, this might not always be a
reasonable assumption. Consider again the motivating example where
each machine in a data center produces streams of measurements. It is desirable to determine
the anomaly score of a data point online as it arrives. The anomaly
measure should be calculated with respect to the data produced so far,
and by a streaming algorithm.
We refer to this as the online scenario. Scores computed in this
setting could be very different from the batch setting. In this work,
we consider both these kinds of measures. Note that the measures
$L^k(i)$ and $T^k(i)$ defined in the introduction are batch
measures, since they assume we know the entire matrix $\Ab$. The
online measures $\ell^k(i)$ and $t^k(i)$ are defined analogously to $L^k(i)$ and $T^k(i)$, except rather than using the entire matrix $\Ab$, we only consider the first $i-1$ rows for the SVD.

\medskip

For both the online and the batch setting, we will work in the
row-streaming model, where each row appears at a point in time. It is
easy to see that there is a trivial $O(d^2)$ memory, $1$-pass
algorithm in the online setting: we maintain the covariance of the
rows seen so far, and use its SVD to computing $\ell^k(i)$ and
$t^k(i)$.

Computing the batch scores in the streaming model
requires care, since even if the rows are seen in streaming order, when
row $i$ arrives, we cannot compute its leverage score without seeing
the rest of the input. Indeed, 1-pass algorithms are not possible
(unless they output the entire matrix of scores at the end of the
pass, which clearly requires a lot of memory).
On the other hand, there is a simple $2$-pass algorithm which uses
$O(d^2)$ memory to compute the covariance matrix in one pass, then
computes its SVD, and using this computes $L^k(i)$ and $T^k(i)$ in a
second pass using memory $O(dk)$. So we could hope for better 2-pass
algorithms.


==> low_rank_approx.tex <==
\section{Low rank approximation using random projections}

\begin{theorem}
		%Consider any matrix $\Ab\in \mathbb{R}^{n\times d}$. Let $\Rb\in \mathbb{R}^{k \times n}$ be a JL matrix such that each entry is an i.i.d. $\tau^2/k$ sub-Gaussian random variable. Define $\Bb =\Rb \Ab$. 
		Consider any matrix $\Ab \in \mathbb{R}^{n \times d}$. Let $\Xb$ be a random matrix with each entry being an i.i.d. sub-Gaussian random variable. Let $\Rb = (1/\sqrt{k})\Xb$, $\Bb = \Rb \Ab$ and assume $\Rb$ is a JL matrix. Let $\{\wb,i\in [k]\}$ be the set the right singular vectors of $\Bb$. Let $\tilde{\Ab}_p=  \sum_{i=1}^{p} (\Ab\wb) \wb_i^T$ be a rank-$p$ approximation of $\Ab$ obtained via the top $p$ right singular vectors of $\Bb$. Then for any $p\le n$ and  $k\ge O\Big(\frac{\bar{\eta}_p+\log(1/\delta)}{\epsilon^4}\Big)$, with failure probability $\delta$,
		\[
		\normfsq{\Ab-\tilde{\Ab}_p} \le \normfsq{\Ab-{\Ab}_p} + {\epsilon}\normfsq{\Ab_p}
		\]
\end{theorem}
\begin{proof}
	We can write $\Ab$, $\Ab_p$ and $\tilde{\Ab}_p$ in terms of the singular value decomposition as follows,
	\[
	\Ab = \sum_{i=1}^{n}\sigma_i \ub_i \vb_i^T, \quad \Ab_p = \sum_{i=1}^{p}\sigma_i \ub_i \vb_i^T, \quad \tilde{\Ab}_p = \sum_{i=1}^{p} (\Ab\wb) \wb_i^T
	\]
	Since $\{\wb_i,i\in [p] \}$ is an orthonormal set of vectors,
	\[
	\normfsq{\Ab-\tilde{\Ab}_p}=\sum_{i=1}^{n}\norm{(\Ab-\tilde{\Ab}_p)\wb_i}^2
	\]
	Note that, by definition, 
	\[ (\Ab-\tilde{\Ab}_p)\wb_i=\begin{cases} 
	\Ab\wb_i - \Ab\wb_i = 0 & \forall \; i \le k \\
	\Ab\wb_i & \forall \; i > k
	\end{cases}
	\]
	Hence,
	\[
	\normfsq{\Ab-\tilde{\Ab}_p}=\sum_{i=k+1}^{n}\norm{\Ab\wb_i}^2 = \sum_{i=1}^{n}\norm{\Ab\wb_i}^2-\sum_{i=1}^{k}\norm{\Ab\wb_i}^2 = \normfsq{\Ab}-\sum_{i=1}^{k}\norm{\Ab\wb_i}^2
	\]
	Note that $\normfsq{\Ab-{\Ab}_p}=\normfsq{\Ab}-\normfsq{\Ab_p}$, therefore,
	\begin{align}
	\normfsq{\Ab-\tilde{\Ab}_p} = \normfsq{\Ab-{\Ab}_p} + (\normfsq{\Ab_p} - \sum_{i=1}^{p}\norm{\Ab\wb_i}^2) \label{eq:low_rank_error}
	\end{align}
	Lemma \ref{lem:low_rank_lem} lower bounds $\sum_{i=1}^{p}\norm{\Ab\wb_i}^2$ ---
	\begin{restatable}{lemma}{lowranklem}\label{lem:low_rank_lem}
				Consider any matrix $\Ab \in \mathbb{R}^{n \times d}$. Let $\Xb$ be a random matrix with each entry being an i.i.d. sub-Gaussian random variable. Let $\Rb = (1/\sqrt{k})\Xb$, $\Bb = \Rb \Ab$ and assume $\Rb$ is a JL matrix. Let $\{\wb,i\in [k]\}$ be the set the right singular vectors of $\Bb$. Let $\tilde{\Ab}_p=  \sum_{i=1}^{p} (\Ab\wb) \wb_i^T$ be a rank-$p$ approximation of $\Ab$ obtained via the top $p$ right singular vectors of $\Bb$. Then for an absolute constant $C$, any $p\le n$ and  $k\ge O\Big(\frac{\bar{\eta}_p+\log(1/\delta)}{\epsilon^4}\Big)$, with failure probability $\delta$,
				\[
				\sum_{i=1}^{p}\norm{\Ab \wb_i}^2 \ge (1-\epsilon)\sum_{i=1}^{p}\sigma_i^2
				\]
	\end{restatable}
	Using Lemma \ref{lem:low_rank_lem}, it follows that,
		\[
		\normfsq{\Ab-\tilde{\Ab}_p} \le \normfsq{\Ab-{\Ab}_p} + {\epsilon}\normfsq{\Ab_p}
		\]

==> notation.tex <==
\section{Notation}

For any matrix $\Ab\in \mathbb{R}^{n\times d}$ having singular values $\{\sigma_i, i \in[n]\}$, we define its $p$-th numeric rank $\eta_p$ as $\eta_p=\normfsq{A}/(\sum_{i=1}^{p}\sigma_i^2/p)$. 

==> online.tex <==
\section{Pointwise guarantees for Anomaly Detection}

\subsection{The Online Setting}\label{sec:online}

We consider the scenario where the rows $\rowa{i} \in \R^d$ arrive in
streaming order. Let $\Ab \in \R^{(i-1) \times d}$ denote the matrix of
points that have arrived so far (excluding $\rowa{i}$) and let $\Ub
\Sigmab \Vb^T$ be its SVD. Write $\rowa{i}$ in the basis of right
singular vectors as $\rowa{i} = \sum_{j = 1}^d\alpha_jv^{(j)}$. We
define its rank-$k$ leverage score and projection distance
respectively as
\begin{align}
 \ell^k(i) & = \sum_{j = 1}^k \frac{\alpha_j^2}{\sigma_j^2} = \sqnorm{\Sigmab_k^{-1}\Vb^T_k\rowa{i}},\label{eq:l-onl}\\
 t^k(i) & = \sum_{j = k+1}^d \alpha_j^2 = \rowa{i}^T(\Ib -\Vb_k\Vb^T_k)\rowa{i}.\label{eq:t-onl}
\end{align}

Let us note that there is a one-pass streaming algorithm that can
compute both these scores on the fly, using time $O(d^3)$ time per
row. We maintain the $d \times d$ covariance matrix $\Ab^T\Ab$and
compute its SVD to get $\Vb_k, \Sigmab_k$. From these, it is easy to
compute both $\ell^k$ and $t^k$.

To approximate these scores, it is natural to use a
sketch $\td{\Ab} \in R^{\ell \times d}$ that approximates the covariance matrix $\Ab^T\Ab$.
We can work with any sketch that guarantees
\begin{align}
  \label{eq:cov}
  \norm{\Ab^T\Ab - \td{\Ab}^T\td{\Ab}} \leq \mu \sigma_1^2.
\end{align}
Given such a sketch, our approximation is the following: compute $\td{\Ab} =
\td{\Ub}\td{\Sigmab}\td{\Vb}^t$. The estimates for $\ell^k(i)$ and $t^k(i)$ respectively are
\begin{align}
  \td{\ell}^k(i) &  = \sqnorm{\td{\Sigmab}_k^{-1}\td{\Vb}^T_k\rowa{i}},\label{eq:lt-onl}\\
  \td{t}^k(i) &  = \rowa{i}^T(\Ib -\tilde\Vb_k\tilde\Vb^T_k)\rowa{i}.\label{eq:tt-onl}
\end{align}

Given the sketch $\td{Ab}$, we can expect that $\td{Vb}_k$ is a
good approximation to the row space spanned by $\Vb_k$, since the
covariance matrices of the rows are close. In contrast the
columns spaces of $\Ab$ and $\td{\Ab}$ are hard to compare since they
lie in $\R^n$ and $\R^\ell$ respectively. The closeness of the row
spaces follows from the results from Section \ref{sec:prelims} but
applied to $\Ab^T$ rather than $\Ab$ itself. The results there require that  $\norm{\Ab\Ab^T -
  \td{\Ab}\td{\Ab}^T}$ is small, and Equation \eqref{eq:cov} implies that
this assumption holds for $\Ab^T$.

We first state our approximation guarantees for $t^k$.

\begin{theorem}
  \label{thm:t-online}
  Assume that $\Ab$ is $(k, \Delta)$-separated. Let $\eps <1/3$ and let $\td{\Ab}$ satisfy
  Equation \eqref{eq:cov} for $\mu = \eps^2\Delta$. Then for every $i$,
  \begin{align*}
    |t^k(i) - \td{t}^k(i)| \leq \eps\sqnorm{\rowa{i}}.
  \end{align*}
\end{theorem}
\begin{proof}
  We have
  \begin{align*}
    |t^k(i) - \td{t}^k(i)| & = |\rowa{i}^T(\Ib -\Vb_k\Vb^T_k)\rowa{i} -
    \rowa{i}^T(\Ib - \tilde{\Vb}_k\tilde{\Vb}^T_k)\rowa{i}| \\
    & = |\rowa(i)(\tilde{\Vb}_k\tilde{\Vb}^T_k -
    \Vb_k\Vb_k^T)\rowa{i}| \\
    & \leq \norm{\tilde{\Vb}_k\tilde{\Vb}^T_k - \Vb_k\Vb_k^T}  \sqnorm{\rowa{i}}\\
    & \leq \eps \sqnorm{\rowa{i}}
  \end{align*}
  where in the last line we use Lemma \ref{lem:wed}, applied to the
  projection onto columns of $\Ab^T$, which are the rows of $\Ab$. The condition
  $\mu < \Delta/6$ holds since $\eps < 1/3$.
\end{proof}


How meaningful is the above additive approximation guarantee? For each
row, the additive error is $\eps\sqnorm{\rowa{i}}$. It might be
that $t^k(i) \ll \eps\sqnorm{\rowa{i}}$ which happens when the row is
almost entirely within the principal subspace. But in this case the,
the points are not anomalies, and we have $\td{t}^k(i) \leq 2\eps
\sqnorm{\rowa{i}}$, so these points will not seem anomalous from the approximation either.
The interesting case is when $t^k(i) \geq \beta \sqnorm{\rowa{i}}$ for
some constant $\beta$ (say $1/2$). For such points, we have
$\td{t}^k(i) \in (\beta \pm \epsilon)\sqnorm{\rowa{i}}$, so we
indeed get multiplicative approximations.

Next we give our approximation guarantee for $\ell^k$.



\begin{theorem}
  \label{thm:l-online}
  Assume that $\Ab$ is $(k, \Delta)$-separated. Let
  \begin{align}
    \eps \leq \min(\kappa\Delta, \frac{1}{k})\sr(\Ab)\kappa. \label{eq:ugly-1}
  \end{align}
  Let $\td{\Ab}$ be as in Equation \eqref{eq:cov} for
  \begin{align}
        \mu = \frac{\eps^3k^2}{10^3 \sr(A)^3\kappa^4} \label{eq:ugly-2}
  \end{align}
  Then for every $i$,
  \begin{align}
    |t^k(i) - \td{t}^k(i)| \leq \eps k
    \frac{\sqnorm{\rowa{i}}}{\|\Ab\|_F^2}. \label{eq:l-guarantee}
  \end{align}
\end{theorem}
\begin{proof}
  We will show that
      \begin{align}
      \norm{\Vb_k\Sigmab_k^{-2}\Vb_k^T - \tilde{\Vb_k}\tilde{\Sigmab}^{-2}\tilde{\Vb}_k^T}
      \leq \frac{\eps k}{\|\Ab\|_F^2}\label{eq:mhnbs}.
      \end{align}
  To prove inequality \eqref{eq:mhnbs}, we will bound the LHS as
  \begin{align}
    \norm{\Vb_k\Sigmab^{-2}\Vb_k^T -
      \tilde{\Vb}_k\tilde{\Sigmab}^{-2}\tilde{\Vb}_k^T} \leq
    \norm{\Vb_k\Sigmab_k^{-2}\Vb_k^T - \tilde{\Vb}_k^T\Sigmab_k^{-2}\tilde{\Vb}_k^T} +
    \norm{\tilde{\Vb}_k(\Sigmab^{-2} - \tilde{\Sigmab}^{-2})\tilde{\Vb}_k^T}\label{eq:mhnbs-0}.
  \end{align}
  For the first term, we apply Lemma \ref{lem:sigma2} to $\Ab^T$ to get
  \begin{align}
    \norm{\Vb_k\Sigmab^{-2}\Vb_k^T -
      \tilde{\Vb}_k^T\Sigmab_k^{-2}\tilde{\Vb}_k^T} \leq
    \frac{8}{\sigma_k^2}(\mu k \kappa)^{1/3}. \label{eq:mhnbs-1}
  \end{align}
  We bound the second term as
  \begin{align}
        \norm{\tilde{\Vb}_k(\Sigmab^{-2} -
          \tilde{\Sigmab}^{-2})\tilde{\Vb}_k^T} & =
        \max_{i \in [k]}|\sigma_i^{-2} - \tilde{\sigma}_i^{-2}|\notag\\
        & = \max_{i \in [k]}\frac{|\sigma_i^2 -
          \tilde{\sigma}_i^2|}{\sigma_i^2\tilde{\sigma}_i^2}\notag\\
        & \leq \frac{\mu\sigma_1^2}{\sigma_k^2\tilde{\sigma}_k^2}\notag\\
        & \leq \frac{2\mu\sigma_1^2}{\sigma_k^4}  =  \frac{2\mu \kappa}{\sigma_k^2}\label{eq:mhnbs-2}
  \end{align}
  where we use Weyl's inequality to bound $\sigma_i^2 -
  \tilde{\sigma}_i^2$ and again to bound
  \[ \tilde{\sigma}_k^2 \geq \sigma_k^2 - \mu\sigma_1^2 \geq
  \sigma_k^2 - \sigma_k^2/10 k \geq \sigma_k^2/2\]
  using $\mu \geq 1/(20k\kappa)$.
  Plugging Equations \eqref{eq:mhnbs-1} and \eqref{eq:mhnbs-2} into
  Equation \eqref{eq:mhnbs-0} gives
    \begin{align}
    \norm{\Vb_k\Sigmab^{-2}\Vb_k^T -
      \tilde{\Vb}_k\tilde{\Sigmab}^{-2}\tilde{\Vb}_k^T} & \leq
    \frac{1}{\sigma_k^2}(8(\mu k \kappa)^{1/3} + 2\mu \kappa) \leq
    \frac{10}{\sigma_k^2}(\mu k \kappa)^{1/3}\label{eq:use-lemma}\\
    & \leq \frac{10}{\sigma_k^2}
    (\frac{\eps^3k^3}{10^3\sr(\Ab)^3\kappa^3})^{1/3}\nonumber\\
    & \leq \frac{k\eps}{\sigma_k^2\kappa \sr(\Ab)} = \frac{k \eps}{\|\Ab\|_F^2}.\nonumber
    \end{align}
    Equation \eqref{eq:use-lemma} follows by Lemma \ref{lem:sigma2}.
    The conditions on $\mu$ needed for that lemma to apply are
    guaranteed by Equation \eqref{eq:ugly-1}.
\end{proof}

To interpret this guarantee, consider the setting when all the points
have roughly the same $2$-norm. More precisely, if for some constant $C$
\[ \frac{\sqnorm{\rowa{i}}}{\|\Ab\|_F^2} \leq \frac{C}{i} \]
then Equation \eqref{eq:l-guarantee} gives
  \begin{align*}
    |t^k(i) - \td{t}^k(i)| \leq C\eps \frac{k}{i}.
  \end{align*}
  Note that $k$ is a constant whereas $i$ grows as more points come
  in. Points which are considered outliers are those where $t^k(i)
\gg \frac{k}{i}$, indeed if a point is truly orthogonal to the points
seen so far, its leverage score is $1$.

For the parameters setting, if we let $\kappa =O(1)$ and $\sr(A) =
\Theta(k)$, then Equation \eqref{eq:ugly-1} reduces to $\eps \leq
\min(\Delta, 1/k)$, and Equation \eqref{eq:ugly-2} to $\mu \approx \eps^3/k$.

To efficiently compute a sketch that satisfies \eqref{eq:cov}, we can use Frequent
Directions \citep{liberty2013simple,Liberty16}, which gives the
following guarantee:
\begin{theorem}\label{thm:fd}
	\citep{Liberty16}
	There is an algorithm that takes the rows of $\Ab$ in
	streaming fashion and computes a sketch $\td{\Ab} \in \R^{\ell
		\times d}$ satisfying Equation \eqref{eq:cov} where $\ell =
	\sum_{i = k+1}^n\sigma_i^2/(\sigma_1^2 \mu)$.
\end{theorem}
Let $\td{\Ab} = \td{\Ub}\td{\Sigmab}\td{\Vb}^T$.
The algorithm  maintains $\td{\Sigmab}, \td{\Vb}$. It uses
$O(d\ell)$ memory and requires time at most $O(d\ell^2)$ per row. The
total time for processing $n$ rows is $O(nd\ell)$. If  $\ell \ll d$,
this is a significant improvement over the naive one-pass algorithm in
both memory and time. If we use Frequent directions, we set
\begin{align}
  \label{eq:fd}
  \ell = \frac{\sum_{i= k+1}^d\sigma_i^2}{\sigma_1^2\eps^2\Delta}
  \leq \frac{\sr(\Ab)}{\eps^2\Delta}
  \end{align}
which is considerably smaller than $d$ for parameter settings of
interest.


\subsection{The batch setting}

In the batch setting, we consider the scenario where the entire matrix
$\Ab \in \R^{n \times d}$ is given as input. Let $\Ub \Sigmab \Vb^T$ be its SVD.
Write $\rowa{i}$ in the basis of right singular vectors as $\rowa{i} =
\sum_{j = 1}^d\alpha_jv^{(j)}$. We define its rank-$k$ leverage score and projection distance
respectively as
\begin{align}
 L^k(i) & = \sum_{j = 1}^k \frac{\alpha_j^2}{\sigma_j^2} = \sqnorm{\Sigmab_k^{-1}\Vb^T_k\rowa{i}},\label{eq:l-onl}\\
 T^k(i) & = \sum_{j = k+1}^d \alpha_j^2 = \rowa{i}^T(\Ib -\Vb_k\Vb^T_k)\rowa{i}.\label{eq:t-onl}
\end{align}
The difference from the online setting is that the SVD is computed for
the entire input. The measure $L^k(i)$ is exactly the row leverage
score for $\rowa{i}$.

Using the same approach as the previous section, we can get a more
efficient algorithm by using a sketch $\td{\Ab}$ of the matrix
$\Ab$. In the first pass, we compute $\td{\Ab}$ using Frequent
Directions and at the end of the pass, we use it to compute
$\Sigmab_k$ and $\Vb_k$. In the second pass, we use these to compute
$L^k$ and $T^k$.The space used is $O(d\ell)$ where $\ell$ is given by
Equation \eqref{eq:fd}, while the update time per row is
$O(d\ell^2)$.

The $\Omega(d)$ lower bounds in Section \ref{sec:lower} suggest that
one cannot hope for sublinear dependence on $\ell$ for pointwise
estimates. In the next section, we suggest an approach which could
potentially eliminate the dependence on $d$ in exchange for weaker guarantees.


==> summary.tex <==
\subsection{Assumptions about the input}

For a matrix $A \in R^{n \times d}$, let $a_{(i)}$ denote its $i^{th}$
row, $a^{(j)}$ denote its $j^{th}$ column. We view each row $a_{(i)}$
as a point in $d$-dimensional space. We will work in the row-streaming
model where the rows arrive one after the other. We assume that $n \gg d$.
Let $A = U \Sigma V^t$ denote its singular value decomposition, where $\Sigma = diag(sigma_1,
\ldots, \sigma_d)$.

For outlier detection, we are interested in the case when the data are approximately low-dimensional.
A natural formalization of approximate low-dimensionality is that a large fraction of the Frobenius norm comes from the top
$k$ singular values:
\begin{Def}
  We say that a matrix $A$ is $(k,\mu)$-concentrated for $\mu \in
  [0,1]$ if
  \begin{align}
    \sum_{i=1}^k \sigma_i^2 & \geq mu \cdot \sum_{i=1}^n \sigma_i^2
  \end{align}
This implies for instance that the numeric rank is bounded:
\begin{Fact}
If $A$ is $(k, \mu)$-concentrated, then $\strk(A) \leq k/\mu$.
\end{Fact}
In particular,  when $\mu \geq 1/2$, we have $\strk(A) \leq 2k$.


In general, there might be multiple $k$-dimensional subspaces that approximate the data. This
arises from degeneracy in the spectrum of the matrix: if $\sigma_k^2 =
\sigma_{k+1}^2$, there can be several $k$-dimensional subspaces
that approximate the data. This is problematic for outlier detection,
since several commonly used measures of anomaly depend on the
principal $k$-dimensional subspace. If this subspace is not well
defined, then neither is the measure. Indeed, this suggests that a
different value of $k$ might be appropriate.

To rule out such degeneracies, we require that $k$ is such that there
is a gap in the spectrum at $k$, which ensures that the principal
subspace is well defined.
\begin{Def}
We say a matrix is $(k, \eta)$-separated if
  \begin{align}
    \sigma_k^2 - \sigma^2_{k+1} \geq \eta
  \end{align}
\end{Def}

We can write a row of the matrix in the basis of right singular
vectors as $a_{(i)} = \sum_{j=1}^d \alpha^i_j v^{(j)}$. We will refer
to the projection onto the $k$-dimensional principal subspace
$a^h_{(i)} = \sum_{j=1}^k \alpha_jv^{(j)}$ as the head and
$a^t_{(i)} = \sum_{j=k+1}^n \alpha_jv^{(j)}$ as the tail.
Our separation assumption ensures these are well defined.


\subsection{Anomaly measures}


The goal of anomaly detection is when a new data point arrives, to assign it an anomaly
score that measures how anomalous it is. There are a wide number of measures of how outlying a point is,
perhaps the most well-studied among them are the statistical leverage
scores, and the closely related Mahalanobis distance. The
leverage score of the $i^{th}$ row is the $2$-norm of the $i^{th}$ row
of $U$:
\[ \ell(i) \defeq \sum_{j=1}^du_{ij}^2.\]
Alternately, if we write the row $a_{(i)} = \sum_{j=1}^d \alpha^i_jv^{(j)}, then
\[ \ell(i) = \sum_{j=1}^d \frac{\alpha^i_j^2}{\sigma_j^2}.\]

If the singular values in the tail are small, (which would be the case
if they come from noise) the above measure will be dominated by the
tail. This motivates the use of separate measures for the head and the tail:
\begin{itemize}
  \item Compare the projection onto the principal
    subspace with the data seen so far. This is (only) concerned with
    the head.
  \item Measure how far from the principal subspace the point
    lies. This measure is (only) concerned with the tail.
\end{itemize}

For the head, we use the rank-$k$ leverage score of $a_{(i)}$ is
\[ \ell^k(i) = \sum_{j=1}^ku_{ij}^2 = \sum_{j=1}^k \frac{\alpha_j^2}{\sigma_j}^2.\]
We will measure deviation in the tail by the distance from the
principal $k$-dimensional subspace, given by
\[ t^{> k}(i)= \sum_{j = k+1}^n\alpha_j^2.\]
We prefer this to using
\[ \ell^{> k}_i \defeq \sum_{j= k + 1}^n \frac{\alpha_j^2}{\sigma_j}^2\]
since it is more robust to the precise value of the small $\sigma_j$, and is seemingly easier to compute in
the streaming setting. \footnote{although the latter measure is also studied in
the literature and may be preferred in settings where there is
structure in the tail}

An alternative approach might be to consider the ridge leverage
scores, which effectively replace the covariance matrix of $A^tA$
with $A^tA + \lambda I$, which increases all the singular values by
$\lambda$, with the effect of damping the effect of small singular
values. We have
\[ \ell_\lambda(i) = \sum_{j=1}^d \frac{\alpha_j^2}{\sigma_j^2 + \lambda}.\]

Consider the case when the data is generated from a true
$k$-dimensional distribution, and then corrupted with a small amount of
white noise. It is easy to see that the data points
will satisfy both concentration and separation
assumptions. In this case, all the notions suggested above will
essentially converge. In this case, we expect $\sigma_{k+1}^2 \approx \cdots
\approx \sigma_n^2$. So
\[ \ell^{> k}_i = \sum_{j= k + 1}^n \frac{\alpha_j^2}{\sigma_j}^2
\approx \frac{t^{> k}(i)}{\sigma_{k+1}^2}. \]
If $\lambda$ is chosen so that $\sigma^2_{k} \gg \lambda \gg \sigma_{k+1}^2$, it follows that
\[ \ell_\lambda(i) \approx \ell^k(i) + \frac{t^{>k}(i)}{\lambda}. \]

\subsection{Our Results}

The main message in this paper is that a small random projection of the input
data points suffices for to compute an efficient approximation of the
outlier measures mentioned above.
The dimension of the sketch can be independent of both $n$ and $d$, under the
assumptions that the data are $(k, \mu)$-concentrated and $(k,
\eta)$-separated, the projection dimension depends only on $k, \mu,
\eta$, provided we are willing to settle for average-case rather than
pointwise guarantees. Combined with the Frequent
directions algorithm for streaming SVD, the resulting scheme lends itself to fast,
memory-efficient computation in the streaming model.


The guarantees we get are of the from
\[ \sum_{i =1}^n|\ell^k(i) - \hat{\ell}^k(i)| \leq \frac{\eps k}{n}. \]
Comparing this with the standard bound
\[ \sum_{i =1}^n\ell^k(i) \leq \frac{k}{n}, \]
we conclude that the avergae outlier score is preserved within $(1+
\eps)$.

